PopNet: Real-Time Population-Level Disease Prediction with Data Latency

Population-level disease prediction estimates the number of potential patients of particular diseases in some location at a future time based on (frequently updated) historical disease statistics. Existing approaches often assume the existing disease statistics are reliable and will not change. However, in practice, data collection is often time-consuming and has time delays, with both historical and current disease statistics being updated continuously. In this work, we propose a real-time population-level disease prediction model which captures data latency (PopNet) and incorporates the updated data for improved predictions. To achieve this goal, PopNet models real-time data and updated data using two separate systems, each capturing spatial and temporal effects using hybrid graph attention networks and recurrent neural networks. PopNet then fuses the two systems using both spatial and temporal latency-aware attentions in an end-to-end manner. We evaluate PopNet on real-world disease datasets and show that PopNet consistently outperforms all baseline disease prediction and general spatial-temporal prediction models, achieving up to 47% lower root mean squared error and 24% lower mean absolute error compared with the best baselines.

==> reviews.tex <==
Reviewer1 (Weak reject):
1.  First, I have a serious concern about its experimental setup, since the detailed information of the dataset is shadowed (i.e. data quantity, metadata distribution). It is highly desirable to have statistics of the datasets. Otherwise, it is hard to evaluate that the experimental setting is proper or not.

2. Second, it is preferable to have some detailed analysis for the ablation studies. Instead of simply offering some quantitative results, more qualitative results may enable us to evaluate both the strengths and weaknesses of each component in the model effectively and bring us deeper insights on how to adapt its method to different real scenarios.

3. Third, the model architecture consists of a pipeline from existing models (i.e. GAT and RNN), so the novelty is weak. Besides, fusing multiple GATs and RNNs incurs high model complexity. Such a model may require high computational resources and prone to be overfitting to the training data, especially when the quantity of the training data is insufficient in some clinical cases.

4. Moreover, the dataset is split by different periods in the Q1 experiment section, but data from different periods may induce different data distribution, which may increase the model variance. To be more specific, the best validation checkpoint represents the most accurate model from April 2019 to July 2019. However, we cannot ensure its generalization ability on the test set which comes from August 2019 to December 2019, because disease statistics will change over time.

5. Lastly, please have your submission proof-read for English style and grammar issues, especially in the introduction section. For example, the graph attention network should be abbreviated as “GAT” instead of “GNN”, and the sequencing word “Second” should be preceded by “First”. Based on these factors, I would vote for rejecting it.

Reviewer2 (Neutral)
1. From the definition 1 and definition 2, it seems that disease statistics data and updated disease data are obtained from two diverse time periods, and how to guarantee the latter one is reliable and can reflect the change of the same location and similar diseases. Besides, what is the reason that the historical disease statistics is not reliable and accurate.

2.How to obtain the temporal latency and what is the different compared to the distance from disease statistics data to updated disease data.

3.What is \hat{a}_ij in Eq. (8) and what is the function.

4.For the ablation methods, such as PopNet-GAT, PopNet-GRU, how to conduct input for the different considerations.

Reviewer 3 (Weak reject):
 1. The authors claim that some statistics are not reliable due to the delayed updates. However, if a disease massively outbreaks at one location, the statistics should be roughly consistent with the statistical information at another location after a period of time, such as case-fatality ratios of COVID19 among states in the US. The authors try to use two variants, PopNet-GAT and PopNet-GRU to prove the importance of considering both spatial and temporal information in the experiments. However, it's interesting to see that PopNet-GRU (No temporal information considered) performs badly (nearly the second-worst performance in disease prediction tasks). Does this mean temporal information is more important than spatial? Meanwhile, I am not convinced that a combination of both factors could achieve the best performance given the bad performance of PopNet-GAT.

2. Why are the regression metrics used for disease prediction? Normally, it’s a classification problem that uses accuracy, AUC, etc. as metrics.


Revewer 4 (Weak reject):
This a well-written paper with a thorough explanation of the method. It integrates multiple techniques in order to address an important problem - spatio-temporal prediction with data latency and data updates. The integration of the techniques gives impressive performance gains. The source code is available allowing practitioners to potentially adopt this method. However, a weakness of the paper is the lack of a conceptual novelty, rather offering integration of several techniques GAT+RNN to drive the performance.

Comments
1. MAE might be insufficient as a metric for data that rapidly changes over brief periods of time since it is decreased through averaging over time. It is necessary to look at maximum error or similar, and perhaps plot the performance over periods of rapid changes in the data.

2. Discussion around Figure 2 (comparison vs. baseline) should attempt to identify or hypothesize the sources of improvement vs. baseline. Eg. why is pregnancy so much better predicted with the algorithm?

Suggestions:
* More datasets: The datasets represent fairly stable processes such as tumors; it would be valuable to evaluate the performance on a say a synthetic dataset of an influenza outbreak which includes sharp peaks and inflection points.

* Location graph on Page 2 "is computed based on the geographical proximity between locations". In reality, there might be strong correlations between locations of say urban centers even when those are far apart (e.g. NY and LA).
* p2 "netowrks" typo.


